Eudoxus: Characterizing and Accelerating Localization in Autonomous Machines

We develop and commercialize autonomous machines, such as logistic robots and self-driving cars, around the globe. A critical challenge to our -- and any -- autonomous machine is accurate and efficient localization under resource constraints, which has fueled specialized localization accelerators recently. Prior acceleration efforts are point solutions in that they each specialize for a specific localization algorithm. In real-world commercial deployments, however, autonomous machines routinely operate under different environments and no single localization algorithm fits all the environments. Simply stacking together point solutions not only leads to cost and power budget overrun, but also results in an overly complicated software stack. This paper demonstrates our new software-hardware co-designed framework for autonomous machine localization, which adapts to different operating scenarios by fusing fundamental algorithmic primitives. Through characterizing the software framework, we identify ideal acceleration candidates that contribute significantly to the end-to-end latency and/or latency variation. We show how to co-design a hardware accelerator to systematically exploit the parallelisms, locality, and common building blocks inherent in the localization framework. We build, deploy, and evaluate an FPGA prototype on our next-generation self-driving cars. To demonstrate the flexibility of our framework, we also instantiate another FPGA prototype targeting drones, which represent mobile autonomous machines. We achieve about 2x speedup and 4x energy reduction compared to widely-deployed, optimized implementations on general-purpose platforms.

==> ack.tex <==
\section{Acknowledgement}

We thank the anonymous reviewers from MICRO 2020  and HPCA 2021 for their valuable feedback and/or guidance. Shaoshan Liu is the corresponding author of the paper. This work is partially funded by an Arm research award and the University Research Award from University of Rochester.


==> exp.tex <==
\section{Experimental Setup}
\label{sec:exp}

\paragraph{Hardware Platform} To show the flexibility and general applicability of our design framework, we build two instances of \proj: one targeting mobile robots and drones using a Zynq \fixme{Ultrascale+} SoC, which integrates an ARM Cortex-A9 CPU with an FPGA on the same chip through the AXI interface, and the other that targets self-driving vehicles, which uses a desktop Intel CPU connected with a dedicated \fixme{Kintex} FPGA board through the PCI-e interface.
%The two platforms differ in the performance and energy constraints, and require different front-end and back-end algorithms.

\paragraph{Dataset} We use two widely-used datasets: KITTI Odometry~\cite{??} for self-driving cars and EuRoC~\cite{??} for drones. \fixme{our dataset?}

\paragraph{Baselines} What baselines do we compare against? 1) GPU baseline of each localization algorithm; 2) accelerator baseline of each localization algorithm; 3) a hypothetical platform that integrates three localization accelerators (mainly for power/resource/area comparisons).

On FPGA unused resources still consume non-trivial idle power so if we were to implement three distinct localization accelerator on an FPGA I'd expect the power overhead to be high, in addition to the high resource usage. Maybe we can show that by using our framework we are able to use a much smaller FPGA (Zynq vs. Ultrascale?), which in itself saves power and reduces cost.







==> impl.tex <==
\section{The \proj System}
\label{sec:sys}

%\label{sec:bedesign}
%\begin{figure}[t]
%\centering
%\includegraphics[width=.6\columnwidth]{sys}
%\caption{System overview.}
%\label{fig:sys}
%%\vspace{15pt}
%\end{figure}

Building on top of the frontend and backend architectures, we describe the complete \proj localization system stack. We choose to build the accelerator on FPGA because of its flexibility and to demonstrate a working system.

%2) the backend mode switching (\Sect{sec:be:design}), 
\paragraph{Hardware} The FPGA accelerates the frontend and the three backend kernels while leaving the rest of the algorithm to the CPU, which mainly executes two components: 1) the runtime scheduler (\Sect{sec:algo:framework}), and 2) the unaccelerated backend code (i.e., all except Projection in \Fig{fig:reg_be_var}, all except Kalman Gain in \Fig{fig:vio_be_var}, and all except Marginalization in \Fig{fig:slam_be_var}), which are lightweight and have little variation.
%Much of the unaccelerated backend code is undergoing frequent updates \fixme{data?}.

%We present a high-level configuration interface to the developers so that they are hidden from the algorithmic details such as the backend modes and mode switching. Specifically, the developers specify the camera, GPS, and IMU frequencies, 

The FPGA is directly interfaced with the cameras and IMU/GPS sensors. The host and the FPGA accelerator communicate three times in each frame: the first time from the FPGA, which transfers the frontend results and the IMU/GPS samples to the host; the second time from the host, which passes the inputs of a backend kernel (e.g., the $\mathbf{H}$, $\mathbf{P}$, and $\mathbf{R}$ matrices to calculate Kalman gains) to the FPGA, and the last time transferring the backend results back to the host.

\paragraph{Software} As mentioned at the end of \Sect{sec:algo:framework}, our software framework directly uses the code building blocks from the dedicated algorithms' open-source implementations, i.e., bag-of-words for registration~\cite{dbow2}, MSCKF for VIO~\cite{msckfvio}, and VINS-Fusion for SLAM~\cite{vinsfusion}. Our algorithm has the same accuracy as the state-of-the-art dedicated algorithms in each mode and is about 4\% faster than each dedicated algorithm due to the removal of ROS dependencies.

%Maybe this is where we can talk a little bit about considerations in practical implementations, i.e., some low-level details that arise in real-world deployment and that are ignored by academics?
%
%\subsection{Software Interface}
%\label{sec:runtime:sw}
%
%We can talk a bit about the software interface. This is not crazily new so I think we can downplay it. Maybe introduce the programming interface in the context that the runtime is hidden from programmers, who use high-level APIs to trigger localization. We provide a set of low-level APIs to probe the system and implement the runtime.
%
%\subsection{Integration}
%\label{sec:runtime:int}
%
%It's important to discuss how our localization system is integrated into the bigger system. Any bottlenecks?

==> related.tex <==
\section{Related Work}
\label{sec:related}

In an unmapped environment, two major classes of algorithms exist: 1) constrained optimization-based approaches~\cite{mur2017orb, engel2014lsd, pumarola2017pl} and 2) probabilistic estimation-based filtering approaches~\cite{marchetti2006comparative, mourikis2007multi, jetto1999development, mao2007design}. In a mapped environment, registration against the map is most effective~\cite{mur2017orb, mur2015orb}. We show that different scenarios require different algorithms, and propose a unified localization software framework, which provides a desirable software target for acceleration.
%, and is usually included as part of many SLAM solutions, known as track against map or re-localization

Compared to prior localization accelerators on ASIC~\cite{suleiman2019navion, li2019879gops, yoon2010graphics} and FPGA~\cite{zhang2017visual, zhang2018pirvs, liu2019eslam, fang2017fpga, gautier2019fpga, boikos2016semi, tertei2016fpga}, \proj differ in three key ways. First, we provide a unified accelerator substrate for different localization algorithms that are required in different environments. We show that simply stacking dedicated accelerators built for each algorithm (the N.S. columns in \mbox{\Tbl{tbl:fpga}}) leads to over 2$\times$ resource waste. Second, \proj characterizes and optimizes not only the average latency, but also latency variation. Finally, with the same design principle, \proj can be instantiated differently to target different autonomous machines with varying performance requirements and constraints, e.g., drones vs. self-driving cars, as we demonstrate in \mbox{\Sect{sec:eval}}.

Broadly, architectural support for autonomous machines has received increasing attention lately, ranging from accelerating motion planning and control~\cite{sacks2018robox, murray2016microarchitecture, murray2016robot}, enabling distributed cognition~\cite{hadidi2018distributed, merck2019characterizing, hadidi2019understanding}, to benchmarking~\cite{weisz2016robobench, boroujerdian2018mavbench, slambench}. This paper particularly focuses on localization.

%Architecture community has also been looking at how to achieve real-time localization using hardware support. Both dedicate hardware design ~\cite{,} and FPGA acceleration ~\cite{} are discussed in literatures. Instead of building one single chip or integrate all the system onto a FPGA board, we choose to dynamically offload the time consuming computation part and high variation procedure onto FPGA board which could save chip area and achieve high efficiency as well.

%Also, compared with achieving one solution on one platform such as robots~\cite{sileshi2016particle}, autonomous driving systems~\cite{nitta2018study} and drones~\cite{vsovstaric2019drone}, \proj can be implemented into different instances with the same design principle. 
